A Unified Graph Language Model for Multi-Domain Multi-Task Graph Alignment Instruction Tuning

Leveraging Graph Neural Networks (GNNs) as graph encoders and aligning the resulting representations with Large Language Models (LLMs) through alignment instruction tuning has become a mainstream paradigm for constructing Graph Language Models (GLMs), combining the generalization ability of LLMs with the structural modeling capacity of GNNs. However, existing GLMs that adopt GNNs as graph encoders largely overlook the problem of aligning GNN-encoded representations across domains and tasks with the LLM token space to obtain unified graph tokens, thereby limiting their ability to generalize across diverse graph data. To bridge this gap, we aim to incorporate a multi-domain, multi-task GNN encoder into GLMs and align its representations with LLMs to enable multi-domain, multi-task graph alignment instruction tuning. This alignment problem remains underexplored and poses two key challenges: 1) learning GNN-encoded representations that are simultaneously generalizable across domains and tasks and well aligned with textual semantics is difficult, due to substantial variations in graph structures, feature distributions, and supervision signals, together with the lack of textual-semantic alignment guidance in task-specific GNN training; 2) diverse graph data and task-specific instructions can exhibit different degrees of compatibility with the LLM token space during instruction tuning, leading to varying alignment difficulty and rendering a fixed alignment strategy suboptimal. To tackle these challenges, we propose UniGraphLM, a Unified Graph Language Model that incorporates a multi-domain, multi-task GNN encoder to learn generalizable graph representations aligned with textual semantics, and then adaptively aligns these representations with the LLM.

==> tables/notation.tex <==


\begin{table*}[!htb]
    \caption{Summary of notations used in this paper.}
    \label{tab:notation}
    \centering
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{ll}
        \toprule
        \textbf{Notation} & \textbf{Description} \\
        \midrule
        $\mathcal{D}$ & Set of graph datasets (domains) used in this work. \\
        $D$ & A dataset/domain, $D\in\mathcal{D}$. \\
        $\mathcal{S}$, $s$ & Domain space and a domain label. \\
        $\mathcal{T}$, $t$ & Task-type space and a task type (node/edge/graph). \\
        $\mathcal{G}_s$ & Graph instance space for domain $s$. \\
        $\mathcal{Y}_t$ & Label/output space for task type $t$. \\
        $\{(G_i, y_i)\}_{i=1}^{N_D}$ & Labeled graph-task instances in dataset $D$; $N_D$ is the number of instances. \\
        $G_i=(\mathcal{V}_i, \mathcal{E}_i, \mathbf{X}_i, \mathbf{E}_i)$ & $i$-th graph instance (nodes, edges, node features, edge features). \\
        $\mathcal{V}_i$, $\mathcal{E}_i$ & Node set and edge set of $G_i$. \\
        $\mathbf{X}_i$, $\mathbf{E}_i$ & Node features and edge features of $G_i$. \\
        $\mathrm{GNN}^{\text{multi}}_{\phi}(\cdot)$, $\phi$ & Multi-scale GNN encoder and its parameters. \\
        $\mathbf{h}_i$, $\mathbf{h}_i^{\ast}$ & Graph representation and task-specific representation at granularity $\ast\in\{\text{node, edge, graph}\}$. \\
        $\mathrm{Project}_{\theta}(\cdot)$, $\theta$ & Projector to the LLM embedding space and its parameters. \\
        $\mathbf{z}_i$ (or $\mathbf{z}_i^{\ast}$) & Graph token(s) after projection, used as part of the LLM input. \\
        $I_i=[\mathbf{q}_i;\mathbf{z}_i;\mathbf{t}_i]$ & Graph-conditioned instruction sequence. \\
        $\mathbf{q}_i$ & Natural-language instruction/query tokens. \\
        $\mathbf{t}_i$ & Target output token sequence corresponding to $y_i$. \\
        $\mathcal{L}$ & Training objective (next-token prediction loss). \\
        $\mathcal{D}_{\text{gt}}=\{(G_i, T_i)\}_{i=1}^{N}$ & Graph-text pair dataset; $T_i$ is the textual description. \\
        $\mathbf{T}_i$ & Text representation encoded from $T_i$ (e.g., Sentence-BERT). \\
        $\mathbf{S}^{g\rightarrow t}$ & Graph-to-text similarity matrix used in contrastive pretraining. \\
        $d_i$ & Domain index (dataset ID) of instance $i$. \\
        $W^{g}_{ab}$, $W^{s}_{ab}$ & Domain-aware weights for negative samples (graph/text side). \\
        $\mathcal{B}_k$ & Mini-batch at optimization step $k$. \\
        $\mathcal{D}_k$ & Active domains appearing in $\mathcal{B}_k$. \\
        $L_i$, $L_D^{(k)}$ & Per-instance loss and aggregated loss for domain $D$ at step $k$. \\
        $g_D^{(k)}$ & Alignment difficulty score for domain $D$ (gradient norm). \\
        $w_D^{(k)}$ & Curriculum weight for domain $D$ at step $k$. \\
        $\tau$ & Temperature in the softmax weighting. \\
        \bottomrule
        \end{tabular}%
    }
\end{table*}
